How Can Recommender Systems Benefit from Large Language Models: A Survey

With the rapid development of online services, recommender systems (RS) have become increasingly indispensable for mitigating information overload. Despite remarkable progress, conventional recommendation models (CRM) still have some limitations, e.g., lacking open-world knowledge, and difficulties in comprehending users' underlying preferences and motivations. Meanwhile, large language models (LLM) have shown impressive general intelligence and human-like capabilities, which mainly stem from their extensive open-world knowledge, reasoning ability, as well as their comprehension of human culture and society. Consequently, the emergence of LLM is inspiring the design of recommender systems and pointing out a promising research direction, i.e., whether we can incorporate LLM and benefit from their knowledge and capabilities to compensate for the limitations of CRM. In this paper, we conduct a comprehensive survey on this research direction from the perspective of the whole pipeline in real-world recommender systems. Specifically, we summarize existing works from two orthogonal aspects: where and how to adapt LLM to RS. For the WHERE question, we discuss the roles that LLM could play in different stages of the recommendation pipeline, i.e., feature engineering, feature encoder, scoring/ranking function, user interaction, and pipeline controller. For the HOW question, we investigate the training and inference strategies, resulting in two fine-grained taxonomy criteria, i.e., whether to tune LLM or not, and whether to involve conventional recommendation models for inference. Then, we highlight key challenges in adapting LLM to RS from three aspects, i.e., efficiency, effectiveness, and ethics. Finally, we summarize the survey and discuss the future prospects. We actively maintain a GitHub repository for papers and other related resources: https://github.com/CHIANGEL/Awesome-LLM-for-RecSys/.

==> github.md.backup.tex <==
Feature Engineering

| **Name** | **Paper** | **LLM Backbone (Largest)** | **LLM Tuning Strategy** | **Publication** | **Link** |
|:---:|:---|:---:|:---:|:---:|:---:|
| GReaT | Language Models are Realistic Tabular Data Generators | GPT2-medium (355M) | Full Finetuning | ICLR 2023 | [[Link]](https://arxiv.org/abs/2210.06280) |
| ONCE | ONCE: Boosting Content-based Recommendation with Both Open- and Closed-source Large Language Models | ChatGPT | Frozen | WSDM 2024 | [[Link]](https://arxiv.org/abs/2305.06566) |
| AnyPredict | AnyPredict: Foundation Model for Tabular Prediction | ChatGPT | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2305.12081) |
| LLM4KGC | Knowledge Graph Completion Models are Few-shot Learners: An Empirical Study of Relation Labeling in E-commerce with LLMs | PaLM (540B)/ ChatGPT | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2305.09858v1) |
| TagGPT | TagGPT: Large Language Models are Zero-shot Multimodal Taggers | ChatGPT | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2304.03022v1) |
| ICPC | Large Language Models for User Interest Journeys | LaMDA (137B) | Full Finetuning/ Prompt Tuning | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2305.15498) |
| DPLLM | Privacy-Preserving Recommender Systems with Synthetic Query Generation using Differentially Private Large Language Models | T5-XL (3B) | Full Finetuning | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2305.05973) |
| KAR | Towards Open-World Recommendation with Knowledge Augmentation from Large Language Models | ChatGPT | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2306.10933) |
| MINT | Large Language Model Augmented Narrative Driven Recommendations | GPT3 (175B) | Frozen | RecSys 2023 | [[Link]](https://arxiv.org/abs/2306.02250) |
| PIE | Product Information Extraction using ChatGPT | ChatGPT | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2306.14921) |
| LGIR | Enhancing Job Recommendation through LLM-based Generative Adversarial Networks | GhatGLM (6B) | Frozen | AAAI 2024 | [[Link]](https://arxiv.org/abs/2307.10747) |
| GIRL | Generative Job Recommendations with Large Language Model | BELLE (7B) | Full Finetuning | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2307.02157) |
| LLM-Rec | LLM-Rec: Personalized Recommendation via Prompting Large Language Models | text-davinci-003 | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2307.15780) |
| HKFR | Heterogeneous Knowledge Fusion: A Novel Approach for Personalized Recommendation via LLM | ChatGPT | Frozen | RecSys 2023 | [[Link]](https://arxiv.org/abs/2308.03333) |
| LLaMA-E | LLaMA-E: Empowering E-commerce Authoring with Multi-Aspect Instruction Following | LLaMA (30B) | LoRA | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2308.04913) |
| EcomGPT | EcomGPT: Instruction-tuning Large Language Models with Chain-of-Task Tasks for E-commerce | BLOOMZ (7.1B) | Full Finetuning | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2308.06966) |
| Agent4Rec | On Generative Agents in Recommendation | ChatGPT | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2310.10108) |
| TF-DCon | Leveraging Large Language Models (LLMs) to Empower Training-Free Dataset Condensation for Content-Based Recommendation | ChatGPT | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2310.09874) |
| RLMRec | Representation Learning with Large Language Models for Recommendation | ChatGPT | Frozen | WWW 2024 | [[Link]](https://arxiv.org/abs/2310.15950) |
| LLMRec | LLMRec: Large Language Models with Graph Augmentation for Recommendation | ChatGPT | Frozen | WSDM 2024 | [[Link]](https://arxiv.org/pdf/2311.00423.pdf) |
| LLMRG | Enhancing Recommender Systems with Large Language Model Reasoning Graphs | GPT-4 | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2308.10835) |
| CUP | Recommendations by Concise User Profiles from Review Text | ChatGPT | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2311.01314) |
| SINGLE | Modeling User Viewing Flow using Large Language Models for Article Recommendation | ChatGPT | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2311.07619) |
| RecPrompt | RecPrompt: A Prompt Tuning Framework for News Recommendation Using Large Language Models | GPT4 | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2312.10463) |
| PO4ISR | Large Language Models for Intent-Driven Session Recommendations | ChatGPT | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2312.07552) |
| Agent4Ranking | Agent4Ranking: Semantic Robust Ranking via Personalized Query Rewriting Using Multi-agent LLM | ChatGPT | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2312.15450) |
| SAGCN | Understanding Before Recommendation: Semantic Aspect-Aware Review Exploitation via Large Language Models | Vicuna (13B) | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2312.16275) |
| UEM | User Embedding Model for Personalized Language Prompting | FLAN-T5-base (250M) | Full Finetuning | Arxiv 2024 | [[Link]](https://arxiv.org/abs/2401.04858) |
| LLMHG | LLM-Guided Multi-View Hypergraph Learning for Human-Centric Explainable Recommendation | GPT4 | Frozen | Arxiv 2024 | [[Link]](https://arxiv.org/abs/2401.08217) |
| Llama4Rec | Integrating Large Language Models into Recommendation via Mutual Augmentation and Adaptive Aggregation | LLaMA2 (7B) | Full Finetuning | Arxiv 2024 | [[Link]](https://arxiv.org/abs/2401.13870) |





| **Name** | **Paper** | **LLM Backbone (Largest)** | **LLM Tuning Strategy** | **Publication** | **Link** |
|:---:|:---|:---:|:---:|:---:|:---:|
| U-BERT | U-BERT: Pre-training User Representations for Improved Recommendation | BERT-base (110M) | Full Finetuning | AAAI 2021 | [[Link]](https://ojs.aaai.org/index.php/AAAI/article/view/16557) |
| UNBERT | UNBERT: User-News Matching BERT for News Recommendation | BERT-base (110M) | Full Finetuning | IJCAI 2021 | [[Link]](https://www.ijcai.org/proceedings/2021/462) |
| PLM-NR | Empowering News Recommendation with Pre-trained Language Models | RoBERTa-base (125M) | Full Finetuning | SIGIR 2021 | [[Link]](https://arxiv.org/abs/2104.07413) |
| Pyramid-ERNIE | Pre-trained Language Model based Ranking in Baidu Search | ERNIE (110M) | Full Finetuning | KDD 2021 | [[Link]](https://arxiv.org/abs/2105.11108) |
| ERNIE-RS | Pre-trained Language Model for Web-scale Retrieval in Baidu Search | ERNIE (110M) | Full Finetuning | KDD 2021 | [[Link]](https://arxiv.org/abs/2106.03373) |
| CTR-BERT | CTR-BERT: Cost-effective knowledge distillation for billion-parameter teacher models | Customized BERT (1.5B) | Full Finetuning | ENLSP 2021 | [[Link]](https://neurips2021-nlp.github.io/papers/20/CameraReady/camera_ready_final.pdf) |
| ZESRec | Zero-Shot Recommender Systems | BERT-base (110M) | Frozen | Arxiv 2021 | [[Link]](https://arxiv.org/abs/2105.08318) |
| UniSRec | Towards Universal Sequence Representation Learning for Recommender Systems | BERT-base (110M) | Frozen | KDD 2022 | [[Link]](https://arxiv.org/abs/2206.05941) |
| SuKD | Learning Supplementary NLP Features for CTR Prediction in Sponsored Search | RoBERTa-large (355M) | Full Finetuning | KDD 2022 | [[Link]](https://dl.acm.org/doi/abs/10.1145/3534678.3539064) |
| PREC | Boosting Deep CTR Prediction with a Plug-and-Play Pre-trainer for News Recommendation | BERT-base (110M) | Full Finetuning | COLING 2022 | [[Link]](https://aclanthology.org/2022.coling-1.249/) |
| MM-Rec | MM-Rec: Visiolinguistic Model Empowered Multimodal News Recommendation | BERT-base (110M) | Full Finetuning | SIGIR 2022 | [[Link]](https://dl.acm.org/doi/abs/10.1145/3477495.3531896) |
| Tiny-NewsRec | Tiny-NewsRec: Effective and Efficient PLM-based News Recommendation | UniLMv2-base (110M) | Full Finetuning | EMNLP 2022 | [[Link]](https://arxiv.org/abs/2112.00944) |
| PLM4Tag | PTM4Tag: Sharpening Tag Recommendation of Stack Overflow Posts with Pre-trained Models | CodeBERT (125M) | Full Finetuning | ICPC 2022 | [[Link]](https://arxiv.org/abs/2203.10965) |
| TwHIN-BERT | TwHIN-BERT: A Socially-Enriched Pre-trained Language Model for Multilingual Tweet Representations | BERT-base (110M) | Full Finetuning | Arxiv 2022 | [[Link]](https://arxiv.org/abs/2209.07562) |
| TransRec | TransRec: Learning Transferable Recommendation from Mixture-of-Modality Feedback | BERT-base (110M) | Full Finetuning | Arxiv 2022 | [[Link]](https://arxiv.org/abs/2206.06190) |
| VQ-Rec | Learning Vector-Quantized Item Representation for Transferable Sequential Recommenders | BERT-base (110M) | Frozen | WWW 2023 | [[Link]](https://arxiv.org/abs/2210.12316) |
| IDRec vs MoRec | Where to Go Next for Recommender Systems? ID- vs. Modality-based Recommender Models Revisited | BERT-base (110M) | Full Finetuning | SIGIR 2023 | [[Link]](https://arxiv.org/abs/2303.13835) |
| TransRec | Exploring Adapter-based Transfer Learning for Recommender Systems: Empirical Studies and Practical Insights | RoBERTa-base (125M) | Layerwise Adapter Tuning | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2305.15036) |
| LSH | Improving Code Example Recommendations on Informal Documentation Using BERT and Query-Aware LSH: A Comparative Study | BERT-base (110M) | Full Finetuning | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2305.03017v1) |
| TCF | Exploring the Upper Limits of Text-Based Collaborative Filtering Using Large Language Models: Discoveries and Insights | OPT-175B (175B) | Frozen/ Full Finetuning | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2305.11700) |
| LLM2BERT4Rec | Leveraging Large Language Models for Sequential Recommendation | text-embedding-ada-002 | Frozen | RecSys 2023 | [[Link]](https://arxiv.org/abs/2309.09261) | 
| LLM4ARec | Prompt Tuning Large Language Models on Personalized Aspect Extraction for Recommendations | GPT2 (110M) | Prompt Tuning | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2306.01475) |
| TIGER | Recommender Systems with Generative Retrieval | Sentence-T5 | Frozen | NIPS 2023 | [[Link]](https://arxiv.org/abs/2305.05065) |
| TBIN | TBIN: Modeling Long Textual Behavior Data for CTR Prediction | BERT-base (110M) | Frozen | DLP-RecSys 2023 | [[Link]](https://arxiv.org/abs/2308.08483) |
| LKPNR | LKPNR: LLM and KG for Personalized News Recommendation Framework | LLaMA2 (7B) | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2308.12028) |
| SSNA | Towards Efficient and Effective Adaptation of Large Language Models for Sequential Recommendation | DistilRoBERTa-base (83M) | Layerwise Adapter Tuning | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2310.01612) |
| S&R Foundation | An Unified Search and Recommendation Foundation Model for Cold-Start Scenario | ChatGLM (6B) | Frozen | CIKM 2023 | [[Link]](https://arxiv.org/abs/2309.08939) |
| CollabContext | Collaborative Contextualization: Bridging the Gap between Collaborative Filtering and Pre-trained Language Model | Instructor-XL (1.5B) | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2310.09400) |
| LMIndexer | Language Models As Semantic Indexers | T5-base (223M) | Full Finetuning | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2310.07815) |
| MISSRec | MISSRec: Pre-training and Transferring Multi-modal Interest-aware Sequence Representation for Recommendation | CLIP-B/32 (400M) | Full Finetuning | MM 2023 | [[Link]](https://arxiv.org/abs/2308.11175) |
| Stack | A BERT based Ensemble Approach for Sentiment Classification of Customer Reviews and its Application to Nudge Marketing in e-Commerce | BERT-base (110M) | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2311.10782) |
| N/A | Utilizing Language Models for Tour Itinerary Recommendation | BERT-base (110M) | Full Finetuning | PMAI@IJCAI 2023 | [[Link]](https://arxiv.org/abs/2311.12355) |
| UFIN | UFIN: Universal Feature Interaction Network for Multi-Domain Click-Through Rate Prediction | FLAN-T5-base (250M) | Frozen | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2311.15493) |
| PMMRec | Multi-Modality is All You Need for Transferable Recommender Systems | RoBERTa-large (355M) | Top-2-layer Finetuning | ICDE 2024 | [[Link]](https://arxiv.org/abs/2312.09602) |
| Uni-CTR | A Unified Framework for Multi-Domain CTR Prediction via Large Language Models | Sheared-LLaMA (1.3B) | LoRA | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2312.10743) |
| UEM | User Embedding Model for Personalized Language Prompting | Sentence-T5-base (223M) | Frozen | Arxiv 2024 | [[Link]](https://arxiv.org/abs/2401.04858) |
| Social-LLM | Social-LLM: Modeling User Behavior at Scale using Language Models and Social Network Data | SBERT-MPNet0base (110M) | Frozen | Arxiv 2024 | [[Link]](https://arxiv.org/abs/2401.00893) |
| LLMRS | LLMRS: Unlocking Potentials of LLM-Based Recommender Systems for Software Purchase | MPNet (110M) | Frozen | Arxiv 2024 | [[Link]](https://arxiv.org/abs/2401.06676) |








    
| **Name** | **Paper** | **LLM Backbone (Largest)** | **LLM Tuning Strategy** | **Publication** | **Link** |
|:---:|:---|:---:|:---:|:---:|:---:|
| TG-ReDial | Towards Topic-Guided Conversational Recommender System | BERT-base (110M) & GPT2 (110M) | Unknown | COLING 2020 | [[Link]](https://arxiv.org/abs/2010.04125) |
| TCP | Follow Me: Conversation Planning for Target-driven Recommendation Dialogue Systems | BERT-base (110M) | Full Finetuning | Arxiv 2022 | [[Link]](https://arxiv.org/abs/2208.03516) |
| BARCOR | BARCOR: Towards A Unified Framework for Conversational Recommendation Systems | BART-base (139M) | Selective-layer Finetuning | Arxiv 2022 | [[Link]](https://arxiv.org/abs/2203.14257) |
| RecInDial | RecInDial: A Unified Framework for Conversational Recommendation with Pretrained Language Models | DialoGPT (110M) | Full Finetuning | AACL 2022 | [[Link]](https://arxiv.org/abs/2110.07477) |
| MESE | Improving Conversational Recommendation Systems' Quality with Context-Aware Item Meta-Information | DistilBERT (67M) & GPT2 (110M) | Full Finetuning | ACL 2022 | [[Link]](https://arxiv.org/abs/2112.08140) |
| UniCRS | Towards Unified Conversational Recommender Systems via Knowledge-Enhanced Prompt Learning | DialoGPT-small (176M) | Frozen | KDD 2022 | [[Link]](https://arxiv.org/abs/2206.09363) |
| UniMIND | A Unified Multi-task Learning Framework for Multi-goal Conversational Recommender Systems | BART-base (139M) | Full Finetuning | ACM TOIS 2023 | [[Link]](https://arxiv.org/abs/2204.06923) |
| VRICR | Variational Reasoning over Incomplete Knowledge Graphs for Conversational Recommendation | BERT-base (110M) | Full Finetuning | WSDM 2023 | [[Link]](https://arxiv.org/abs/2212.11868) |
| KECR | Explicit Knowledge Graph Reasoning for Conversational Recommendation | BERT-base (110M) & GPT2 (110M) | Frozen | ACM TIST 2023 | [[Link]](https://arxiv.org/abs/2305.00783) |
| T5-CR | Multi-Task End-to-End Training Improves Conversational Recommendation | T5-base (223M) | Full Finetuning | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2305.06218) |
| TtW | Talk the Walk: Synthetic Data Generation for Conversational Music Recommendation | T5-base (223M) & T5-XXL (11B) | Full Finetuning & Frozen | Arxiv 2023 | 
| N/A | Rethinking the Evaluation for Conversational Recommendation in the Era of Large Language Models | ChatGPT | Frozen | EMNLP 2023 | [[Link]](https://arxiv.org/abs/2305.13112) |
| N/A | Large Language Models as Zero-Shot Conversational Recommenders | GPT4 | Frozen | CIKM 2023 | [[Link]](https://arxiv.org/abs/2308.10053) |
| MuseChat | MuseChat: A Conversational Music Recommendation System for Videos | Vicuna (7B) | LoRA | Arxiv 2023 | [[Link]](https://arxiv.org/abs/2310.06282) |
| N/A | Conversational Recommender System and Large Language Model Are Made for Each Other in E-commerce Pre-sales Dialogue | Chinese-Alpaca-7B | LoRA | EMNLP 2023 Findings | [[Link]](https://arxiv.org/abs/2310.14626) |

==> sections/introduction.tex <==
\section{Introduction}

With the rapid development of online services, recommender systems (RS) have become increasingly important to match users' information needs~\cite{dai2021adversarial,fu2023f} and alleviate the problem of\xinyi{mitigating} information overload~\cite{guo2017deepfm}. 
\textcolor{blue}{They cast personalized suggestions over a range of candidate items to meet individual preferences in various downstream domains, \eg, e-commerce~\cite{schafer2001commerce}, movie~\cite{goyani2020review}, music~\cite{song2012survey}, etc.}
\xinyi{These systems offer personalized suggestions across diverse domains such as e-commerce, e-commerce~\cite{schafer2001commerce}, movie~\cite{goyani2020review}, music~\cite{song2012survey}, etc}
Despite the different\xinyi{varied} forms of application\xinyi{recommendation} tasks (\eg, top-$N$
recommendation, or sequential recommendation), the common learning objective for a deep learning based\xinyi{remove deep learning based} recommender system is to estimate a given user's preference towards each candidate item, and finally arrange\xinyi{present} a ranked list of items presented to the user~\cite{lin2021graph,xi2023bird}. 

\textcolor{blue}{
Despite the successful progress of conventional recommenders\xinyi{conventional recommender systems (RSs)} over the past decades, their recommendation performance is still suboptimal with limitations coming from two major drawbacks\xinyi{their recommendation performance is still suboptimal, hampered by two major drawbacks.}: 
(1) Conventional RSs are closed systems generally built based on anonymous ID features within a few datasets and domains\xinyi{the specific domians}~\cite{xi2023towards}. Therefore, they lack the open-world commonsense knowledge to obtain better recommendation performance (\eg, enhancing user interest modeling and item content understanding)\xinyi{other?} domains~\cite{harte2023leveraging,liu2023first,chen2023knowledge}. 
(2) Traditional RS is able to achieve promising performance for tasks with simple decisions\xinyi{not decision.}(\eg, click-through rate prediction, rating prediction)~\cite{fan2023recommender}, but they cannot truly understand the underlying preferences and intentions of users for complex scenarios. For example, they might lack recommendation explainability~\cite{gao2023chat,chen2023survey}, and cannot deal with conversational requirements from users~\cite{friedman2023leveraging,wang2022recindial,wang2022barcor}.
}
\xinyi{Conventional RSs often frame recommendation tasks as standard prediction tasks (\eg, click-through rate prediction, rating prediction)~\cite{fan2023recommender}, neglecting the modeling of users' intricate preference and the underlying motivations behind user behaviors, especially in scenarios involving vague preference or deep-seated motivations. As a result, these systems might lack recommendation explainability~\cite{gao2023chat,chen2023survey}, and cannot deal with conversational requirements from users~\cite{friedman2023leveraging,wang2022recindial,wang2022barcor}.}

On the other hand, in the field of natural language processing (NLP), large language model (LLM) has shown impressive emergent abilities (\eg, logical reasoning~\cite{huang2022towards}, in-context few-shot learning~\cite{brown2020language}), as well as the vast reservoir of open-world knowledge compressed in their pretrained model parameters~\cite{zhao2023survey}. 
\xinyi{Large language models implicitly store massive amount of world knowledge in there parameters~\cite{zhao2023survey}, and show remarkable reasoning abilities~\cite{huang2022towards}, which naturally compensate for the aforementioned two drawbacks of Conventional RSs. Therefore, LLMs can be used at various stages of industrial recommendation systems, significantly enhancing the transferability, interpretability, and understanding of complex user intents.}

\textcolor{blue}{Therefore, considering the remarkable breakthroughs of LLM in various deep learning applications and the drawbacks of conventional recommender systems, it is natural to propose the following research question:}
% While LLM is making remarkable breakthroughs in various deep learning applications, it is natural to propose the following research question: 

\vspace{5pt}
\emph{How can recommender systems benefit from large language models for performance enhancements and user experience improvements?}
\vspace{5pt}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{imgs/overallv2.pdf}
    \caption{The decomposition of our core research question about adapting large language models to recommender systems. We analyze the question from two orthogonal perspectives: (1) where to adapt LLM, and (2) how to adapt LLM. Note that CRM stands for conventional recommendation model.}
    \label{fig:overall two perspectives}
\end{figure}

To this end, in this paper, we aim to conduct an in-depth survey on the adaption of large language models to recommender systems. 
\textcolor{blue}{
There exist several related survey works that delve into the potential of LLM for general information systems rather than recommender systems, \eg, personalization~\cite{chen2023large}, user modeling~\cite{tan2023user}, and information retrieval~\cite{chen2023large}.
When it comes to the field of recommender systems, \citet{wu2023survey} conduct a review on both discriminative and generative LLMs for recommendation with different tuning strategies.
\citet{fan2023recommender} focus on the pretraining, finetuning and prompting approaches when leveraging LLM for recommendation. 
Other works also concentrate on one specific aspect of recommender systems with LLM enhancements, \eg, prompting strategy~\cite{xu2024prompting}, generative recommendation~\cite{li2023large}, and explainable recommendation~\cite{chen2023survey}.
\xinyi{None of this works propose a systematic view of the utilization of LLMs on the overall pipeline of an industrial recommender systems, and propose feasible, instructive suggestions for the evolution of existing online recommendation platforms in the era of large language models. }
Different from these related works, this paper mainly study the LLM-enhanced recommender systems from an application view and comprehensively discuss the utilization of LLM on the overall pipeline for industrial recommender phases, which we argue is valuable and instructive for recommender system developments, especially for industrial applications and platforms.
}

\textcolor{blue}{To be specific, as shown in Figure~\ref{fig:overall two perspectives}, we comprehensively analyze the latest research progresses, and decompose the aforementioned research question about LLM-enhanced recommender systems from the following two perspectives:}

% To be specific, we study the research question from an application-oriented view and cover a broad range of the latest research works, which we argue is valuable and instructive for recommender system developments, especially for industrial applications and platforms.
% As shown in Figure~\ref{fig:overall two perspectives}, we comprehensively analyze the latest research progresses, and decompose the research question above from two perspectives:
\begin{itemize}[leftmargin=10pt]
    \item \textbf{``WHERE''} question focuses on where to adapt LLM for RS, and discusses the roles that LLM could play at different parts of the modern deep learning based recommender system pipeline, \ie, feature engineering, feature encoder, scoring/ranking function, user interaction, and pipeline controller.\ljh{figure to be modified: add user interaction}
    \item \textbf{``HOW''} question centers on how to adapt LLM for RS, where two orthogonal taxonomy criteria are carried out: (1) whether we will freeze the parameters of the large language model during the training phase, and (2) whether we will involve conventional recommendation models (CRM) during the inference phase.
\end{itemize}

Moreover, we would like to make two further statements before we move on to the details of this survey paper:
\begin{itemize}[leftmargin=10pt]
    \item To provide a thorough survey and a clear development trajectory, we broaden the scope of large language models, and bring those relatively smaller language models (\eg, BERT~\cite{devlin2018bert}, GPT2~\cite{radford2019language}) into the discussion as well.
    \item We focus on works that leverage LLM together with their pretrained parameters to handle textual features via prompting, and exclude works that simply apply pretraining paradigms from NLP domains to pure ID-based traditional recommendation models (\eg, BERT4Rec~\cite{sun2019bert4rec}). Interested readers can refer to \cite{yu2022self,liu2023pre}.\ljh{Do we need to summarize the contribution? I think NO need}
\end{itemize}

The rest of this paper is organized as follows. 
In Section~\ref{sec:preliminary}, we briefly introduce the background and preliminary for recommender systems and large language models.
Section~\ref{sec: where} and Section~\ref{sec: how} thoroughly analyze the aforementioned taxonomies from two perspectives (\ie, \textbf{``WHERE''} and \textbf{``HOW''}), followed by detailed discussion and analysis of the general development trajectories.
In Section~\ref{sec: challenge}, we highlight five key challenges and future directions for the adaption of LLM to RS from three aspects (\ie, \textbf{efficiency}, \textbf{effectiveness}, and \textbf{ethics}), which mainly arise from the unique characteristics of recommender systems especially in industrial applications.
Finally, Section~\ref{sec:conclusion} concludes this survey and draws a hopeful vision for future prospects in research communities of LLM-enhanced recommender systems.


==> sections/introduction_new.tex <==
\section{Introduction}

With the rapid development of online services, recommender systems (RS) have become increasingly important to match users' information needs~\cite{dai2021adversarial,fu2023f} and mitigate information overload~\cite{guo2017deepfm}. 
They offer personalized suggestions across diverse domains such as e-commerce~\cite{schafer2001commerce}, movie~\cite{goyani2020review}, music~\cite{song2012survey}, etc.
Despite the varied forms of recommendation tasks (\eg, top-$N$ recommendation, and sequential recommendation), the common learning objective for recommender systems is to estimate a given user's preference towards each candidate item, and finally arrange a ranked list of items presented to the user~\cite{lin2021graph,xi2023bird}. 

Despite the successful progress of conventional recommender systems over the past decades, their recommendation performance is still suboptimal, hampered by two major drawbacks: 
(1) Conventional recommender systems are closed systems generally built based on anonymous ID features within specific domains~\cite{xi2023towards}. 
Therefore, they lack open-world commonsense knowledge to obtain better recommendation performance (\eg, enhancing user interest modeling and item content understanding), or even to acquire transferring abilities across different domains and platforms~\cite{harte2023leveraging,liu2023first,chen2023knowledge}. \xx{The purpose of "transferring abilities" is also to obtain better recommendation performance?} 
(2) Conventional recommender systems often frame recommendation tasks as standard prediction tasks (\eg, click-through rate prediction, rating prediction)~\cite{fan2023recommender}, neglecting the modeling of users' intricate preference and the underlying motivations behind user behaviors, especially in scenarios involving vague preference or deep-seated motivations \xx{What are scenarios involving deep-seated motivations ? Or it means scenarios lacking deep motivation?}. As a result, these systems might lack recommendation explainability~\cite{gao2023chat,chen2023survey}, and cannot deal with conversational requirements from users~\cite{friedman2023leveraging,wang2022recindial,wang2022barcor}. 

On the other hand, large language models (LLM) implicitly store massive amount of open-world knowledge in their parameters~\cite{zhao2023survey}, and exhibit impressive emergent abilities (\eg, reasoning~\cite{huang2022towards}, instruction following~\cite{brown2020language} \xx{three examples is better, such as "instruction following, logical reasoning, and problem-solving". Besides, explain how LLM can compensate the second drawback.} ). Hence, the rising of large language models naturally compensate \xx{compensates} for the aforementioned two drawbacks of conventional recommender systems. 
As a result, LLM can be used at various stages of industrial recommender systems, significantly enhancing the transferability, interpretability, and understanding of complex user intents. 

% \textcolor{blue}{Therefore, considering the remarkable breakthroughs of LLM in various deep learning applications and the drawbacks of conventional recommender systems, it is natural to propose the following research question:}
% % While LLM is making remarkable breakthroughs in various deep learning applications, it is natural to propose the following research question: 

% \vspace{5pt}
% \emph{How can recommender systems benefit from large language models for performance enhancements and user experience improvements?}
% \vspace{5pt}

To this end, in this paper, we aim to conduct an in-depth survey on the adaption of large language models to recommender systems. 
% \textcolor{blue}{
There exist several related survey works that delve into the potential of \xx{adapting} LLM for general information systems rather than recommender systems, \eg, personalization~\cite{chen2023large}, user modeling~\cite{tan2023user}, and information retrieval~\cite{chen2023large}.
When it comes to the field of recommender systems, \citet{wu2023survey} conduct a review on both discriminative and generative LLMs for recommendation with different tuning strategies.
\citet{fan2023recommender} focus on the pretraining, finetuning and prompting approaches when leveraging LLM for recommendation. 
Other works also concentrate on one specific aspect of recommender systems with LLM enhancements, \eg, prompting strategy~\cite{xu2024prompting}, generative recommendation~\cite{li2023large}, and explainable recommendation~\cite{chen2023survey}.
Different from the existing survey papers, in this paper, we propose a systematic view of the utilization of LLM on the overall pipeline of industrial recommender systems, and propose feasible and instructive suggestions for the evolution of existing online recommendation platforms in the era of large language models. \xx{Emphasize the importance of real-world applications, which is not mentioned in the previous survey works.}
To be specific, as shown in Figure~\ref{fig:overall two perspectives}, 
we comprehensively analyze the latest research progresses, and propose research questions about LLM-enhanced recommender systems from the following two perspectives:

\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{imgs/overallv2.pdf}
    \caption{The decomposition of our core research question about adapting large language models to recommender systems. We analyze the question from two orthogonal perspectives: (1) where to adapt LLM, and (2) how to adapt LLM. Note that CRM stands for conventional recommendation model.}
    \label{fig:overall two perspectives}
\end{figure}

% To be specific, we study the research question from an application-oriented view and cover a broad range of the latest research works, which we argue is valuable and instructive for recommender system developments, especially for industrial applications and platforms.
% As shown in Figure~\ref{fig:overall two perspectives}, we comprehensively analyze the latest research progresses, and decompose the research question above from two perspectives:
\begin{itemize}[leftmargin=10pt]
    \item \textbf{``WHERE''} question focuses on where to adapt LLM for RS, and discusses the roles that LLM could play at different stages of current recommender system pipeline, \ie, feature engineering, feature encoder, scoring/ranking function, user interaction, and pipeline controller. 
    % \ljh{figure to be modified: add user interaction}
    \item \textbf{``HOW''} question centers on how to adapt LLM for RS, where two orthogonal taxonomy criteria are carried out: (1) whether we will freeze the parameters of the large language model during the training phase, and (2) whether we will involve conventional recommendation models (CRM) during the inference phase.
\end{itemize}

Moreover, we would like to make two further statements before we move on to the details of this survey paper:
\begin{itemize}[leftmargin=10pt]
    \item To provide a thorough survey and a clear development path, we broaden the scope of large language models, and bring those relatively smaller language models (\eg, BERT~\cite{devlin2018bert}, GPT2~\cite{radford2019language}) into the discussion as well.
    \item We focus on works that leverage LLM together with their pretrained parameters to handle textual features via prompting, and exclude works that simply apply pretraining paradigms from NLP domains to pure ID-based traditional recommendation models (\eg, BERT4Rec~\cite{sun2019bert4rec}). Interested readers can refer to \cite{yu2022self,liu2023pre}.
    % \ljh{Do we need to summarize the contribution? I think NO need}\xinyi{agree}
\end{itemize}

The rest of this paper is organized as follows. 
In Section~\ref{sec:preliminary}, we briefly introduce the background and preliminary for recommender systems and large language models.
Section~\ref{sec: where} and Section~\ref{sec: how} thoroughly analyze the aforementioned taxonomies from two perspectives (\ie, \textbf{``WHERE''} and \textbf{``HOW''}), followed by detailed discussion and analysis of the general development path \xx{of what?}.
In Section~\ref{sec: challenge}, we highlight five key challenges and future directions for the adaption of LLM to RS from three aspects (\ie, \textbf{efficiency}, \textbf{effectiveness}, and \textbf{ethics}), which mainly arise from the real-world applications of recommender systems.
% unique characteristics of recommender systems especially in industrial applications.
Finally, Section~\ref{sec:conclusion} concludes this survey and draws a hopeful vision for future prospects in research communities of LLM-enhanced recommender systems.


==> sections/resources.tex <==
\section{Resources}



==> sections/table_section.tex <==
\section{Summary Table}

note that one work might exist in different stages of the pipeline.


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly

% \clearpage
% \onecolumn

% \begin{center}
% \begin{landscape}
% \setlength\LTcapwidth{\textwidth} % default: 4in (rather less than \textwidth...)
% \setlength\LTleft{0pt}            % default: \parindent
% \setlength\LTright{0pt}           % default: \fill
{\small\tabcolsep=3pt  % hold it local
\begin{longtable}{@{}ccccc@{}}
\caption{An organization of works on adapting large language models (LLM) to recommender systems (RS). We use the following abbreviations. \textbf{FFT}: full finetuning. \textbf{PT}: prompt tuning. \textbf{LAT}: layerwise adapter tuning. \textbf{OT}: option tuning. \textbf{T-FEW}: few-shot parameter efficient tuning. Note that only the largest models used in the corresponding papers are listed. If the version of the pretrained language model is not specified, we assume it to be the base version.}
\label{tab:my-table}\\
% \resizebox{\textwidth}{!}{
	% \renewcommand\arraystretch{1.0}
\toprule
\textbf{Model Name} &
  \textbf{LLM Backbone} &
  \textbf{LLM Tuning Strategy} &
  \textbf{RS Task} &
  \textbf{RS Scenario} \\* \midrule
\endfirsthead
%
\multicolumn{5}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\toprule
\textbf{Model Name} &
  \textbf{LLM Backbone} &
  \textbf{LLM Tuning Strategy} &
  % \textbf{\begin{tabular}[c]{@{}c@{}}LLM Tuning \\ Strategy\end{tabular}} &
  \textbf{RS Task} &
  \textbf{RS Scenario} \\* \midrule
\endhead
%
\rowcolor[rgb]{0.949,0.504,0.504}\multicolumn{5}{c}{\textbf{Feature Engineering}} \\* \midrule
GReaT  \cite{borisov2023language} &
  GPT2-Medium (355M) &
  FFT &
  N/A &
  Tabular \\* \midrule
GENRE \cite{liu2023first} &
  ChatGPT &
  Frozen &
  \begin{tabular}[c]{@{}c@{}}Retrieval\\ Sequential RS\end{tabular} &
  News \\* \midrule
AnyPredict \cite{wang2023anypredict} &
  ChatGPT &
  Frozen &
  N/A &
  Tabular \\* \midrule
LLM4KGC \cite{chen2023knowledge} &
  \begin{tabular}[c]{@{}c@{}}PaLM (540B) \\ChatGPT\end{tabular} &
  Frozen &
  N/A &
  E-commerce \\* \midrule
TagGPT \cite{li2023taggpt} &
  ChatGPT &
  Frozen &
  Item Tagging &
  \begin{tabular}[c]{@{}c@{}}Food\\ Video\end{tabular} \\* \midrule
ICPC \cite{christakopoulou2023large} &
  LaMDA (137B)&
  FFT/PT &
  User Profiling &
  N/A \\* \midrule
DPLLM \cite{carranza2023privacy} &
  T5-XL (3B) &
  FFT &
  \begin{tabular}[c]{@{}c@{}}Retrieval\\Privacy\end{tabular} &
  Web Search \\* \midrule
\rowcolor[rgb]{0.582,0.879,0.824}\multicolumn{5}{c}{\textbf{Feature Encoder}} \\* \midrule
U-BERT \cite{qiu2021u} &
  BERT-base (110M) &
  FFT &
  Rating Prediction &
  \begin{tabular}[c]{@{}c@{}}Business\\ E-commerce\end{tabular} \\* \midrule
UNBERT \cite{zhang2021unbert} &
  BERT-base (110M) &
  FFT &
  Sequential RS &
  News \\* \midrule
PLM-NR \cite{wu2021empowering} &
  RoBERTa-base (125M) &
  FFT &
  Sequential RS &
  News \\* \midrule
Pyramid-ERNIE \cite{zou2021pre} &
  ERNIE (110M) &
  FFT &
  Ranking &
  Web Search \\* \midrule
ERNIE-RS \cite{liu2021pre} &
  ERNIE (110M) &
  FFT &
  Retrieval &
  Web Search \\* \midrule
CTR-BERT \cite{muhamed2021ctr} &
  Customized BERT (1.5B) &
  FFT &
  CTR Prediction &
  E-commerce \\* \midrule
ZESRec \cite{ding2021zero} &
  BERT-base (110M) &
  Frozen &
  Sequential RS &
  E-commerce \\* \midrule
UniSRec \cite{hou2022towards} &
  BERT-base (110M) &
  Frozen &
  Sequential RS &
  E-commerce \\* \midrule
PREC \cite{liu2022boosting} &
  BERT-base (110M) &
  FFT &
  CTR Prediction &
  News \\* \midrule
MM-Rec \cite{wu2022mm} &
  BERT-base (110M) &
  FFT &
  Sequential RS &
  News \\* \midrule
Tiny-NewsRec \cite{yu2022tiny} &
  UniLMv2-base (110M) &
  FFT &
  Sequential RS &
  News \\* \midrule
PTM4Tag \cite{he2022ptm4tag} &
  CodeBERT (125M) &
  FFT &
  Top-N RS &
  posts \\* \midrule
TwHIN-BERT \cite{zhang2022twhin} &
  BERT-base (110M) &
  FFT &
  Social RS &
  posts \\* \midrule
VQ-Rec \cite{hou2023learning} &
  BERT-base (110M) &
  Frozen &
  Sequential RS &
  E-commerce \\* \midrule
IDRec  vs MoRec \cite{yuan2023go} &
  BERT-base (110M) &
  FFT &
  Sequential RS &
  \begin{tabular}[c]{@{}c@{}}News\\ Video\\ E-commerce\end{tabular} \\* \midrule
TransRec \cite{fu2023exploring} &
  RoBERTa-base (125M) &
  LAT &
  \begin{tabular}[c]{@{}c@{}}Cross-domain RS\\ Sequential RS\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}News\\ Video\\ E-commerce\end{tabular} \\* \midrule
LSH \cite{rahmani2023improving} &
  BERT-base (110M) &
  FFT &
  Top-N RS &
  Code \\* \midrule

\rowcolor[rgb]{0.836,0.965,0.676}\multicolumn{5}{c}{\textbf{Scoring/Ranking Function (Item Scoring Task)}} \\* \midrule
LMRecSys \cite{zhang2021language} &
  GPT2-XL (1.5B) &
  FFT &
  Top-N RS &
  Movie \\* \midrule
PTab \cite{liu2022ptab} &
  BERT-base (110M) &
  FFT &
  N/A &
  Tabular \\* \midrule
UniTRec \cite{mao2023unitrec} &
  BART (406M) &
  FFT &
  Sequential RS &
  \begin{tabular}[c]{@{}c@{}}News\\ Question\\ Social Media\end{tabular} \\* \midrule
Prompt4NR \cite{zhang2023prompt} &
  BERT-base/110M &
  FFT &
  Sequential RS &
  News \\* \midrule
RecFormer \cite{li2023text} &
  LongFormer/149M &
  FFT &
  Sequential RS &
  Product \\* \midrule
TabLLM \cite{hegselmann2023tabllm} &
  T0 (11B) &
  T-FEW &
  N/A &
  Tabular \\* \midrule
Zero-shot GPT \cite{sileo2022zero} &
  GPT2-Medium (355M) &
  Frozen &
  Rating Prediction &
  Movie \\* \midrule
FLAN-T5 \cite{kang2023llms} &
  FLAN-T5-XXL (11B) &
  FFT &
  Rating Prediction &
  \begin{tabular}[c]{@{}c@{}}Book\\ Movie\end{tabular} \\* \midrule
BookGPT \cite{zhiyuli2023bookgpt} &
  ChatGPT &
  Frozen &
  \begin{tabular}[c]{@{}c@{}}Sequential RS\\ Top-N RS\\ Summary Recommendation\end{tabular} &
  Book \\* \midrule
TALLRec \cite{bao2023tallrec} &
  LLaMA (7B) &
  LoRA &
  Sequential RS &
  \begin{tabular}[c]{@{}c@{}}Book\\ Movie\end{tabular} \\* \midrule
\rowcolor[rgb]{0.836,0.965,0.676}\multicolumn{5}{c}{\textbf{Scoring/Ranking Function (Item Generation Task)}} \\* \midrule
GPT4Rec \cite{li2023gpt4rec} &
  GPT2 (110M) &
  FFT &
  Sequential RS &
  E-commerce \\* \midrule
UP5 \cite{hua2023up5} &
  T5-base (223M) &
  FFT &
  \begin{tabular}[c]{@{}c@{}}Retrieval\\ Sequential RS\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Movie\\ Insurance\end{tabular} \\* \midrule
VIP5 \cite{geng2023vip5} &
  T5-base (223M) &
  LAT &
  \begin{tabular}[c]{@{}c@{}}Sequential RS\\ Top-N RS\\ Explaination Generation\end{tabular} &
  E-commerce \\* \midrule
P5-ID \cite{hua2023index} &
  T5-small (61M) &
  FFT &
  Sequential RS &
  \begin{tabular}[c]{@{}c@{}}Business\\ E-commerce\end{tabular} \\* \midrule
FaiRLLM \cite{zhang2023chatgpt} &
  ChatGPT &
  Frozen &
  Top-N RS &
  \begin{tabular}[c]{@{}c@{}}Music\\ Movie\end{tabular} \\* \midrule
PALR \cite{chen2023palr} &
  LLaMA (7B) &
  FFT &
  Sequential RS &
  \begin{tabular}[c]{@{}c@{}}Movie\\ E-commerce\end{tabular} \\* \midrule
ChatGPT-3 \cite{hou2023large} &
  ChatGPT &
  Frozen &
  Sequential RS &
  \begin{tabular}[c]{@{}c@{}}Movie\\ E-commerce\end{tabular} \\* \midrule
AGR \cite{lin2023sparks} &
  ChatGPT &
  Frozen &
  Conversational RS &
  N/A \\* \midrule
NIR \cite{wang2023zero} &
  GPT-3 (175B) &
  Frozen &
  Sequential RS &
  Movie \\* \midrule
\rowcolor[rgb]{0.836,0.965,0.676} \multicolumn{5}{c}{\textbf{Scoring/Ranking Function (Hybrid Task)}} \\* \midrule
% \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} \\
P5 \cite{geng2022recommendation} &
  T5-base (223M) &
  FFT &
  \begin{tabular}[c]{@{}c@{}}Rating Prediction\\ Top-N RS\\ Sequential RS\\ Explanation Generation\\ Review Summarization\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Business\\ E-commerce\end{tabular} \\* \midrule
M6-Rec \cite{cui2022m6} &
  M6-base (300M) &
  OT &
  \begin{tabular}[c]{@{}c@{}}Retrieval\\ Ranking\\ Explanation Generation\\ Conversational RS\end{tabular} &
  E-commerce \\* \midrule
InstructRec \cite{zhang2023recommendation} &
  Flan-T5-XL (3B) &
  FFT &
  \begin{tabular}[c]{@{}c@{}}Sequential RS\\ Product Search\\ Personalized Search\\ Matching-then-reranking\end{tabular} &
  E-commerce \\* \midrule
ChatGPT-1 \cite{liu2023chatgpt} &
  ChatGPT &
  Frozen &
  \begin{tabular}[c]{@{}c@{}}Rating Prediction\\ Top-N RS\\ Sequential RS\\ Explanation Generation\\ Review Summarization\end{tabular} &
  E-commerce \\* \midrule
ChatGPT-2 \cite{dai2023uncovering} &
  ChatGPT &
  Frozen &
  \begin{tabular}[c]{@{}c@{}}Pointwise Ranking\\ Pairwise Ranking\\ List-wise Ranking\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}News\\ Movie\\ E-commerce\end{tabular} \\* \midrule
ChatGPT-4 \cite{sun2023chatgpt} &
  ChatGPT &
  Frozen &
  Passage Reranking &
  Web Search \\* \midrule
\rowcolor{gray}\multicolumn{5}{c}{\textbf{Pipeline Controller}} \\* \midrule
Chat-REC \cite{gao2023chat} &
  ChatGPT &
  Frozen &
  \begin{tabular}[c]{@{}c@{}} Rating Prediction\\Top-N RS \end{tabular}&
  Movie \\* \midrule
RecLLM \cite{friedman2023leveraging} &
  LLaMA (7B) &
  FFT &
  Conversational RS &
  Video \\* \bottomrule
% }
\end{longtable}
}
